Lightweight Relational Embedding in Task-Interpolated Few-Shot Networks for Enhanced Gastrointestinal Disease Classification

Traditional diagnostic methods like colonoscopy are invasive yet critical tools necessary for accurately diagnosing colorectal cancer (CRC). Detection of CRC at early stages is crucial for increasing patient survival rates. However, colonoscopy is dependent on obtaining adequate and high-quality endoscopic images. Prolonged invasive procedures are inherently risky for patients, while suboptimal or insufficient images hamper diagnostic accuracy. These images, typically derived from video frames, often exhibit similar patterns, posing challenges in discrimination. To overcome these challenges, we propose a novel Deep Learning network built on a Few-Shot Learning architecture, which includes a tailored feature extractor, task interpolation, relational embedding, and a bi-level routing attention mechanism. The Few-Shot Learning paradigm enables our model to rapidly adapt to unseen fine-grained endoscopic image patterns, and the task interpolation augments the insufficient images artificially from varied instrument viewpoints. Our relational embedding approach discerns critical intra-image features and captures inter-image transitions between consecutive endoscopic frames, overcoming the limitations of Convolutional Neural Networks (CNNs). The integration of a light-weight attention mechanism ensures a concentrated analysis of pertinent image regions. By training on diverse datasets, the model's generalizability and robustness are notably improved for handling endoscopic images. Evaluated on Kvasir dataset, our model demonstrated superior performance, achieving an accuracy of 90.1\%, precision of 0.845, recall of 0.942, and an F1 score of 0.891. This surpasses current state-of-the-art methods, presenting a promising solution to the challenges of invasive colonoscopy by optimizing CRC detection through advanced image analysis.

==> chapters/Previous.tex <==
% This guideline points out several endoscopic findings, such as distended appearance, erosion/ulcer, fold convergence, and deformity/stiffness, as diagnostic markers of submucosal deep invasive colorectal cancer. Among these findings, invasive depth stands out as a pivotal feature, with deeper invasion suggesting a higher risk of residual cancer post-endoscopic resection and lymph node metastases \cite{shaukat2020endoscopic}. Specifically, colonoscopy excels in screening the pathology by pinpointing the invasive depth.

ResNet12, an extension of the Residual Network \cite{resnet} (ResNet) architecture, is designed for image classification tasks and is characterized by its depth and the inclusion of skip connections to mitigate the vanishing gradient problem in DNNs. While its 12-layer architecture allows for sophisticated feature extraction from images, several drawbacks are noted, especially in the context of endoscopic image analysis. The increased complexity due to hop connections and the potential for overfitting on small datasets necessitate careful application and may pose challenges in scenarios with limited data and computational resources. Moreover, the complexity of ResNet12 can impede interpretability, a vital aspect in medical applications to ensure the model’s decisions can be transparently scrutinized and validated by healthcare professionals.
